Breaking the Mold: Nonlinear Ranking Function Synthesis Without Templates

This paper studies the problem of synthesizing (lexicographic) polynomial ranking functions for loops that can be described in polynomial arithmetic over integers and reals. While the analogous ranking function synthesis problem for linear arithmetic is decidable, even checking whether a given function ranks an integer loop is undecidable in the nonlinear setting. We side-step the decidability barrier by working within the theory of linear integer/real rings (LIRR) rather than the standard model of arithmetic. We develop a termination analysis that is guaranteed to succeed if a loop (expressed as a formula) admits a (lexicographic) polynomial ranking function. In contrast to template-based ranking function synthesis in real arithmetic, our completeness result holds for lexicographic ranking functions of unbounded dimension and degree, and effectively subsumes linear lexicographic ranking function synthesis for linear integer loops.

==> main-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[\pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Let \begin {align*} \hat {F} &= \algorithmfont {zero-stable-restrict}(F) \\ G_0 &= \algorithmfont {zero-stable-restrict}(G) \ . \end {align*} Since $\hat {F} \models F$ and $F \models G$, we have $\hat {F} \models G$. Since $\hat {F} \models G$, $\hat {F}$ is zero-stable, and $G_0$ is the weakest zero-stable formula that entails $G$, we have $\hat {F} \models G_0$. Since \algorithmfont {terminate-PRF}($G$) = true, $\PRF (G_0)$ is non-empty, and so $\PRF (\hat {F})$ is non-empty, and thus \algorithmfont {terminate-PRF}($F$) = true.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[\pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}We prove by induction that at the start of each iteration in \autoref {alg:lprf}, we always have $F^{(k)} \models G^{(k)}$. The base case $ F^{(0)} = F \models G = G^{(0)}$ is trivial. Now assume the statement is true for $F^{(k)} \models G^{(k)}$. Then their zero-stable restrictions $\hat {F} \models G_0$ by \autoref {lem:zero-stable-restrict-properties}. Thus $\QPRF (\hat {F}) \supseteq \QPRF (G_0)$. Now suppose that \begin {align*} F^{(k+1)} &= F^{(k)} \land \bigwedge _{z_i \in Z} z_i' = z_i \land \bigwedge _{p_j \in P} p_j' = p_j \\ G^{(k+1)} &= G^{(k)} \land \bigwedge _{n_k \in N} n_k' = n_k \land \bigwedge _{m_l \in M} m_l' = m_l \end {align*} For each $n_k$ or $m_l$, it is contained in the set $\QPRF (G_0)$ and therefore is also contained in the set $\QPRF (\hat {F})$. Since all $\QPRF $ of $\hat {F}$ can be written as $\sum _{z_i \in Z} f_i z_i + \sum _{p_j \in P} \lambda _j p_j, f_i \in \mathbb {Q}[X], \lambda _j \in \Qplus $, so does any $n_k$ or $m_l$, Thus $\bigwedge _{z_i \in Z} z_i' = z_i \land \bigwedge _{p_j \in P} p_j' = p_j \models n_k' = n_k \land m_l' = m_l$ for any $n_k$ and $m_l$. And consequently $F^{(k+1)} \models G^{(k+1)}$. Given this, if \autoref {alg:lprf} returns $\true $ for $G$, then for some $G^{(t)}$ it is unsatisfiable modulo $\ThZ $. But $F^{(t)} \models G^{(t)}$ so it must also be unsatisfiable modulo $\ThZ $, and the algorithm will also return $\true $ on input $F$.\end{proof}

